Optimal Rate Sampling in 802.11 Systems

In 802.11 systems, Rate Adaptation (RA) is a fundamental mechanism allowing transmitters to adapt the coding and modulation scheme as well as the MIMO transmission mode to the radio channel conditions, and in turn, to learn and track the (mode, rate) pair providing the highest throughput. So far, the design of RA mechanisms has been mainly driven by heuristics. In contrast, in this paper, we rigorously formulate such design as an online stochastic optimisation problem. We solve this problem and present ORS (Optimal Rate Sampling), a family of (mode, rate) pair adaptation algorithms that provably learn as fast as it is possible the best pair for transmission. We study the performance of ORS algorithms in both stationary radio environments where the successful packet transmission probabilities at the various (mode, rate) pairs do not vary over time, and in non-stationary environments where these probabilities evolve. We show that under ORS algorithms, the throughput loss due to the need to explore sub-optimal (mode, rate) pairs does not depend on the number of available pairs, which is a crucial advantage as evolving 802.11 standards offer an increasingly large number of (mode, rate) pairs. We illustrate the efficiency of ORS algorithms (compared to the state-of-the-art algorithms) using simulations and traces extracted from 802.11 test-beds.

==> non_stat2.tex <==
\section{Non-stationary environments}\label{sec:nonstat}

We extend previous results and algorithms to the case where the radio environement is not stationary, i.e., the transmission success probabilities at various rates evolve over time. We assume that when this evolution is relatively slow, we can design algorithms that track the best rate for transmission efficiently. 

\subsection{Channel models and structural properties}

We first make the following assumption, stating that $\theta(t)$ is a Lipschitz function.

\begin{assumption}\label{as:lip}
$t\mapsto \theta(t)$ is $\sigma$-Lipschitz, for some $\sigma>0$: for any $k=1,\ldots, K$, for any $t,t'$:
$$
|\theta_k(t')-\theta(t)| \le \sigma |t'-t|.
$$
\end{assumption}

Since the optimal rate changes over time, we cannot expect that the average rewards are always well separated and that strict unimodality always holds as stated in Assumption \ref{as:uni}. However, we still assume that the unimodal structure is preserved, and make assumptions about the periods of time where different rates yield very similar throughput. More precisely, in the following analysis, we shall use one of the two following assumptions.

\begin{assumption}\label{assum:separation1}
There exists $\overline{\Delta} > 0$ such that for all $\Delta \leq \overline{\Delta}$:
\eq{
\sum_{n=1}^{T} \sum_{k \neq k^{\star}(n)} \indic \{  | r_k \theta_k(n) -   r_{k^\star(n)} \theta_{k^\star}(n) | < \Delta \} = o(T).
}
\end{assumption}

\begin{assumption}\label{assum:separation2}
For all $\Delta > 0$ we have that:
\eq{
\sum_{n=1}^{T} \sum_{k \neq k^{\star}(n)} \indic \{  | r_k \theta_k(n) -   r_{k^\star(n)} \theta_{k^\star}(n) | < \Delta \} \leq \frac{K T \Delta}{r_1}  +   o(T).
}
\end{assumption}

Assumption~\ref{assum:separation1} means that the proportion of time where the optimal arm is not separated from a non optimal arm is negligible. Assumption~\ref{assum:separation2} is more eralistic, and states that the proportion of time where   ... is satisfied if for all $k$, $n \mapsto \theta_k(n)$ follows a stationary ergodic process with uniform stationery distribution on $[0,1]$.

\subsection{Objective}





\subsection{SW-ORS Algorithm}





	In practice, the values of the $\theta$'s evolve over time, and when they are slowly varying, we may design algorithms that actually {\it track} the evolving optimal rate. MAB problems with non-stationary rewards have received little attention so far, but a natural and efficient way of tracking the changes of $\theta$ is to select the rate at time $t$ based on observations made over a fixed time window preceding $t$, i.e., to account for transmissions that occurred between time $t-\tau$ and $t$, see e.g. \cite{garivier08}. The time window $\tau$ is empirically chosen: it must be large enough (to be able to learn), but small enough so that the channel conditions do not vary significantly during a period of duration $\tau$.

	The success probability of rate $k$ at time $n$ is written $\theta_k(n)$. We will consider a \emph{ slowly varying environnement }, so that the rate of change of the parameters is bounded by a constant $\sigma > 0$. For all $n,n^\prime$ we have the Lipschitz condition:
\eq{	
	| \theta_k(n) - \theta_k(n^\prime) |\leq \sigma | n - n^\prime |.  
}

	The empirical average reward of rate $k$ at time $n$ is then calculated by considering the observed rewards during the time window $[n-\tau,n]$:
\al{
	\hat\mu_{k}(n) &= \frac{1}{t_k(n)} \sum_{ n^\prime = n-\tau }^{n}  r_k X_k(n^\prime) \indic \{k(n^\prime) = k \}  \\
	t_k(n) &=  \sum_{ n^\prime = n-\tau }^{n} \indic \{k(n^\prime) = k \},
}
	where $X_k(n^\prime) = 1$ iff a transmission at rate $k$ was successful at time $n^\prime$. Since $\theta_k(n)$ depends on $n$, it is noted that $\hat\mu_{k}(n)$ is now a \emph{biased} estimator of $r_k \theta_k(n)$. The bias is upper bounded by:
	 \eq{		
	 | r_k \theta_k -  \EE[\hat\mu_{k}(n)]  | \leq r_k \tau \sigma.
	 }	
	
	We will compare the performance of KL-UCB and KL-U-UCB in such an environment. The regret of algorithm $\pi$ in a time varying environment is defined as:
 \eq{		
	R^{\pi}(T) = \sum_{n = 1}^{T} \sum_{k=1}^{K} ( r_{k^\star} \theta_{k^\star}(n) - r_k \theta_k(n)) \PP[ k(n) = k  ].
	 }
	It is noted that since the environment is not stationary, the regret $R^{\pi}(T)$ must depend linearly on $T$. To compare the performance of algorithms, we will consider the \emph{ regret per unit of time} $R^{\pi}(T) / T$.
	\subsection{Asymptotic regret per unit of time of KL-UCB and KL-U-UCB}
	
\begin{theorem}\label{th:KLUCBchanging}
		Consider a time varying environment with rate of change $\sigma$ and window size $\tau$. For all $I_{min} > 0$ and $\epsilon$, the regret of $\pi=$KL-UCB per unit of time is upper bounded by:
	\al{	
		\frac{R^{\pi}(T)}{T}  &\leq  r_K \Lp \sqrt{\frac{I_{min}}{2}} + 2 \tau \sigma \Rp \frac{G(T,I_{min},\tau,\sigma)}{T}  +  K r_K (1 + \epsilon) \frac{\log(\tau) + c \log(\log(\tau)) }{\tau I_{min}} \sk 
		&+  O \Lp \frac{1}{g_0 \epsilon^2  \tau^{1 + g_0 \epsilon^2} (\log(\tau))^{c(1 + g_0 \epsilon^2)-1} I_{min}^2} \Rp + O( T/\tau),
	 }
	with:
	\al{
		G(T,I_{min},\tau,\sigma) \leq  \sum_{n=1}^{T} \sum_{k \neq k^{\star}(n)} & \indic \{  r_k (\theta_k(n) + \tau \sigma) \geq  r_{k^\star(n)} (\theta_{k^\star}(n) - \tau \sigma)  \} \sk & \cup  \{    I(\theta_k(n) + \tau \sigma,  r_{k^\star(n)}(\theta_{k^\star}(n) - \tau \sigma)/r_k  \})  > I_{min} \}
	}
	with  $g_0 = \theta_0(1 - \theta_0)/2$ and $\theta_0 = \sigma \tau + \min_{1 \leq n \leq T} \min_{k \neq k^{\star}(n), \theta_k(n) < 1} \theta_k(n)$.
\end{theorem}

	The quantity $G(T,I_{min},\tau,\sigma)$ is the amount of time, up to time $T$, that there exists at least a $k \neq k^\star(n)$,  which cannot be distinguished from $k^\star(n)$ well enough. Namely, either the difference between the average reward of $k$ and $k^\star(n)$ is smaller than the error caused by the changing environment, or the KL-divergence between them is smaller than a fixed threshold $I_{min}$. 
	
The regret of KL-U-UCB in a slowly changing environment is given by theorem~\ref{th:KLUUCBchanging}.

\begin{theorem}\label{th:KLUUCBchanging}
		Consider a time varying environment with rate of change $\sigma$ and window size $\tau$. For all $I_{min} > 0$, $\Delta > 0$ and $\epsilon > 0$, the regret of $\pi=$KL-U-UCB per unit of time is upper bounded by:
	\al{	
		\frac{R^{\pi}(T)}{T}  &\leq  r_K \Lp \sqrt{\frac{I_{min}}{2}} + 2 \tau \sigma \Rp \frac{G(T,I_{min},\tau,\sigma)}{T}  + r_K \frac{H(T,\Delta,\tau,\sigma)}{T} \sk     
		&+  2 r_K (1 + \epsilon) \frac{\log(\tau) + c \log(\log(\tau)) }{\tau I_{min}} + O(\frac{1}{\tau}),
	 }
	with:
	\al{
		H(T,\Delta,\tau,\sigma) \leq  \sum_{n=1}^{T} \sum_{k =1}^{K} \sum_{ k^{\prime} \in N(k)} & \indic \{  | r_k \theta_k(n) - r_{k^\prime} \theta_{k^\prime}(n) |   \geq   \Delta + 2 r_K \tau \sigma)  \}
	}
\end{theorem}
	The function $H(T,\Delta,\tau,\sigma)$ is the number of time instants at which there is an arm which is not well separated from one of its neighbors.
	
	\subsection{Asymptotic regret per unit of time}
		
	The function $G$ is a characteristic of how the probabilities of success $n \mapsto ( \theta_k(n) )_{1 \leq k \leq K}$. We are interested in the performance of the algorithm in a \emph{slowly} changing environment, so that $\sigma \to 0^+$. In this case, it is logical to choose a large window size $\tau \to +\infty$ and a small threshold $I_{min}$. We are interested in how the regret per unit of time scales with $\sigma$ in the regime $\sigma , I_{min} \to 0^+$ , $\tau \to +\infty$. The scaling depends on the value of $G$ in this regime. $G$ depends on how often the average reward of $k^\star(n)$ is arbitrarily close to the average reward of $k \neq k^\star(n)$. This is related to the ``needle in a haystack'' problem discussed in \cite{Auer2003}. We consider two possible assumptions on $G$.

\begin{assumption}\label{assum:separation1}
	There exists $\overline{\Delta} > 0$ such that for all $\Delta \leq \overline{\Delta}$:
	\eq{
	\sum_{n=1}^{T} \sum_{k \neq k^{\star}(n)} \indic \{  | r_k \theta_k(n) -   r_{k^\star(n)} \theta_{k^\star}(n) | < \Delta \} = o(T).
	}
\end{assumption}

\begin{assumption}\label{assum:separation2}
	For all $\Delta > 0$ we have that:
	\eq{
	\sum_{n=1}^{T} \sum_{k \neq k^{\star}(n)} \indic \{  | r_k \theta_k(n) -   r_{k^\star(n)} \theta_{k^\star}(n) | < \Delta \} \leq \frac{K T \Delta}{r_1}  +   o(T).
	}
\end{assumption}
 Assumption~\ref{assum:separation1} means that the proportion of time where the optimal arm is not separated from a non optimal arm is negligible.
 
 Assumption~\ref{assum:separation2} is satisfied if for all $k$, $n \mapsto \theta_k(n)$ follows a stationary ergodic process with uniform stationery distribution on $[0,1]$.

Propositions~\ref{prop:klucbregret1} and ~\ref{prop:klucbregret2} give the regret per unit of time for assumptions~\ref{assum:separation1} and~\ref{assum:separation2} respectively.

\begin{proposition}\label{prop:klucbregret1}
	With assumption~\ref{assum:separation1}, the regret per unit of time of KL-UCB is:
	\al{
	 \lim \sup_{T} \frac{R^{\pi}(T)}{T}  &\leq  \frac{8 \sigma K r_K^4}{\overline{\Delta}^3} \Lb \log \Lp \frac{\overline{\Delta}}{ 4 \sigma r_K } \Rp + c \log \Lp \log  \Lp \frac{\overline{\Delta}}{ 4 \sigma r_K } \Rp \Rp \Rb + O(\sigma)  \sk
	 &=  O(K \sigma \log(1/\sigma)),
	}
	when choosing $\tau = \frac{\overline{\Delta}}{4 \sigma r_K}$ and $I_{min} = \frac{\overline{\Delta}^2}{2 r_K^2}$. 	
\end{proposition}

\begin{proposition}\label{prop:klucbregret2}
	With assumption~\ref{assum:separation2}, and $c > 1$, the regret per unit of time of KL-UCB is:	
	\al{
	 \lim \sup_{T} \frac{R^{\pi}(T)}{T}  &\leq  \Lp 1 + \frac{1}{\sqrt{2 g_0}} \Rp K r_K \sigma^{\frac{2}{5}} \Lb  \frac{r_K}{r_1} \right. \sk 
	 & \left. +  4 \log \Lp \frac{1}{2 \sigma^{\frac{4}{5}}} \Rp + 4 c \log \Lp \log  \Lp \frac{1}{2 \sigma^{\frac{4}{5}}}  \Rp \Rp + O \Lp \frac{1}{\sqrt{ \log (1/\sigma) } } \Rp \Rb \sk
	 &=  O( K \sigma^{\frac{2}{5}} \log(1 /\sigma)). 
	}
	when choosing $\epsilon = \frac{1}{\sqrt{2 g_0}}$, $\tau = \frac{1}{2 \sigma^{\frac{4}{5}}}$ and $I_{min} = \frac{\sigma^{\frac{2}{5}}}{2}$.
\end{proposition}



==> numOLD.tex <==
\section{Numerical Experiments} \label{sec:num}

In this section, we present numerical results to assess the
performance of the proposed algorithm, and compare it to that obtained
by SampleRate\cite{bicket2005bit}. We first use simulation benchmarks as those used in \cite{bicket2005bit}. Then we test the algorithms against real traces extracted from our indoor test-bed.

\subsection{Simulations}

The algorithms are tested in three different scenarios as
in \cite{bicket2005bit}: {\it Steep}, {\it Gradual}, and {\it Lossy}. In
{\it Steep} scenarios, the transmission success probability at any given
rate is either very high or very low. In {\it Gradual} scenario, the
optimal rate is always the highest rate whose success probability
greater than 0.5. Finally in {\it Lossy} scenario, the optimal rate has
a success probability less than 0.5. We consider 802.11g-like systems
with possible rates equal to 6, 9, 12, 18, 24, 36, 48 and 54 Mbit/s. In all plots,
time is measured in slot, of duration roughly equal to
0.5ms, and regrets are expressed in bits: a point of regret 1 means 0.5kbits.

\smallskip
{\bf \em Tested algorithms.}
 Our plots compare the regrets obtained under SampleRate, KL-R-UCB and KL-U-UCB.
SampleRate keeps a time window and basically adopts the rate that induced the highest throughput during the last time window.
At every tenth packet transmission, SampleRate {\em explores} higher rates; it randomly chooses a rate $r_{new}$ which is higher than the throughput $r_c\hat{\theta}_c$ of current rate $r_c$.
When packet losses are sequentially occured four times, SampleRate does not pick the rate during next time window.
KL-R-UCB operates very similar to KL-U-UCB. However, KL-R-UCB chooses the rate whose index is the highest among all rates, whereas
KL-U-UCB looks only neighboring rates of the leader. The regret induced by KL-R-UCB has the asymptotic lower bound derived in Theorem \ref{th:lower_indep}.

% \subsusection{Stationary environments}
\smallskip
{\bf \em Stationary environments.}
We start with stable radio environments where the success probabilities
do not vary over time. The curves we present correspond to the following
success probabilities: {\sl Steep} $\theta=(0.99, 0.98, 0.96, 0.93, 0.9, 0.1, 0.06, 0.04)$; {\sl
  Gradual} $\theta=(0.95, 0.9, 0.8, 0.65, 0.45, 0.25, 0.15, 0.1)$; {\sl Lossy}
$\theta=(0.9, 0.8, 0.7, 0.55, 0.45, 0.35, 0.2, 0.1)$. All $\theta$ values hold correlations and unimodality, i.e., $\theta\in {\cal T}\cap {\cal U}$.


 Fig.~\ref{fig:logscale} examines the asymptotic optimality of KL-U-UCB. Notice that the slope of C2-Bound is gentler than that of C1-Bound.
This indicates that exploiting correlations and unimodality probably brings significant performance
gains. KL-U-UCB and KL-R-UCB seem to be matched C2-Bound and C1-Bound respectively, and thus
KL-U-UCB outperforms KL-R-UCB. We did not consider
SampleRate in Fig.~\ref{fig:logscale} since its regret scale linearly,
not logarithmically with time. This is partly due to the fact that
SampleRate explores new rates every 10 transmissions.

\begin{figure}[htp]
  \centering
  \subfigure[Steep]{%
  \label{fig:steep_log}
  \includegraphics*[width=0.48\columnwidth]{steep_log.pdf}} \hspace{-3mm}
 \subfigure[Gradual]{
  \label{fig:gradual_log}
  \includegraphics*[width=0.48\columnwidth]{gradual_log.pdf}}
\caption{Regrets vs. $\log$(time). `C1-Bound' and `C2-Bound' correspond to
  $c_1(\theta)\log(T)$ and $c_2(\theta)\log(T)$, respectively.}
  \label{fig:logscale}
\end{figure}

In Fig.~\ref{fig:stationary}, we compare the regrets of the various
algorithms in the three scenarios. The window size of SampleRate has been here optimized, and set to 500. 
SampleRate always has low performance, except initially under in the steep scenario. Remember that
SampleRate decreases the selected rate after 4 consecutive losses, which
is rare in the steep scenario, and hence it performs relatively well
there (the algorithms identifies the optimal rate, and stays there
unless 4 losses occur consecutively). On the other hand, in gradual and
lossy cases, 4 consecutive losses may occur more often, which explains
why SampleRate performs so poorly compared to our algorithms. 

\begin{figure*}[t]
  \centering
  \subfigure[Steep]{
   \label{fig:steep}
  \includegraphics [width=0.3\textwidth ]{steep.pdf}} \hspace{-4mm}
  \subfigure[Gradual]{
  \label{fig:gradual}
  \includegraphics [width=0.3\textwidth ]{gradual.pdf}} \hspace{-4mm}
  \subfigure[Lossy]{
  \label{fig:lossy}
  \includegraphics [width=0.3\textwidth ]{lossy.pdf}}
\vspace{0.1cm}
\caption{Regret vs. time in the three scenarios.}
  \label{fig:stationary}
  \vspace{-0.5cm}
\end{figure*}


%\subsection {Non-stationary environments}
\smallskip
{\bf \em Non-stationary environments.} We examine the regret under
non-stationary environment as well. To do so, we artificially
generated slowly varying success probabilities at the different
rates. Fig.~\ref{fig:mu} presents the evolution of the throughputs at different rates over time. In the beginning, the value of $\theta$ corresponds to a  {\sl
steep} scenario, it then evolves to a gradual and finally in a lossy
scenario. We set the
time horizon to be 20,000 and the size of sliding window is 2,000.
SampleRate perform well in only early phase (steep).
It is shown that when the optimal rate changes (at time around 12,000 and 18,000),
the regrets under all algorithms grow rapidly. As we expected, a sliding window helps a transmitter
to adjust to the variation and leads a moderate increase in the regret around turning points.

\begin{figure}[t!]
  \centering
  \subfigure[Evolution of $r_k\theta_k$]{
  \label{fig:mu}
  \includegraphics*[width=0.48\columnwidth]{mu.pdf}} \hspace{-3mm}
 \subfigure[Regret changes for a non-stationary channel]{
  \label{fig:nonstationary}
  \includegraphics*[width=0.48\columnwidth]{nonst.pdf}}
\caption{Regret vs. time. Non-stationary environment.}
  \label{fig:nonst}
\end{figure}


\subsection {Test-bed experiments}

{\bf \em Measurements setup.}  We construct a small indoor test-bed
consisting of two 802.11g nodes (a transmitter and a receiver) on a floor of a
building and collect the real traces recording the goodputs for 8 rates (6, 9, 12,
18, 24, 36, 48 and 54 Mbps). The two nodes are connected in ad-hoc mode
and our measurements were performed in the late night and early morning to minimize the
external interference. We have tested two kinds of scenarios: (a) first, the respective positions of the transmitter and receiver were fixed, and in this case, we observed that the success transmission probabilities at various rates were not really evolving over time -- this is a stationary environment. (b) Then, we made the receiver move (with the speed of a pedestrian), and this generated a non-stationary environment. In our experiments, the
transmitter sends a series of 1500 bytes
packets to the receiver with a bit rate chosen in round-robin from the
given 8 rates, where the time to transmit a batch of 8 packets
for each rate takes about 10 msec. Each trace records the transmission successes and the
failures for each rate.

% {\bf \em Measurements setup.}
% We construct a small indoor test-bed with
% two 802.11g nodes on a floor of a building and collect the real traces
% of goodputs for 8 rates (6, 9, 12, 18, 24, 36, 48 and 54 Mbps).
% A point-to-point 802.11g network testbed
% was deployed on the same floor of a building. We measured channel
% conditions in two different sceanarios : \emph{stationary} and
% \emph{non-stationary}.  To construct a stationary channel, two nodes
% were force to be stayed during measurements. On the other hand, we
% carried one node and slowly move around the other node to see a
% non-stationary channel condition.  We considered 8 bit-rates (6, 9, 12,
% 18, 24, 36, 48 and 54 Mbps) for which OFDM is used as a modulation
% scheme in 802.11g .  In our experiment, one node transmits 1500-byte udp
% packets to the other node with changing the bit-rate in a round robin
% manner, i.e., one packet is sent at 6Mbps, the next packet is sent at
% 9Mbps, and so on.  The required time to transimit a batch of 8 packets
% at each different rates is about 10ms.  We recorded all informations
% about successes or failures of transmissions at each rate and we compare
% the performance of the proposed algorithms with SampleRate algorithm
% using the data traces.

\smallskip {\bf \em Results.}  

Fig.~\ref{fig:st_trace} and
\ref{fig:nonst_trace} show the goodput traces ($r_k\theta_k$) for each
rate, measured over 300 seconds, for stationary and non-stationary
scenarios, respectively. We see that the plots in Fig.~\ref{fig:st_trace} are ``flat'', while those in Fig.~\ref{fig:nonst_trace} show slow variations due to mobility.

We first confirmed the validity of correlation and unimodality assumptions for success probabilities at several transmission rates.
Although we display only two traces in this paper (Fig.~\ref{fig:st_trace} and
\ref{fig:nonst_trace}), we obtained more than fifty 300-seconds-long real traces and checked that those properties are satisfied in all traces.
For example, in case of Fig.~\ref{fig:st_trace}, throughput goes up as the rate rises up to 36Mbps but throughput becomes to decline at higher bit-rates.  


In Fig.~\ref{fig:st_result}, we show how, in the stationary scenario, the instantaneous throughputs averaged over 10 s evolve over time for the different algorithms.
We also put the `Oracle' algorithm which always knows the best rate so that we know how far our proposed algorithm is from the best possible algorithm. 


% transmission at each rate for 300 seconds.
%$\theta_k$ is calculated by considering transmissions during the last 10 seconds.
% The curves in Fig. \ref{fig:st_trace} are relatively flat, i.e., $\theta_k$'s hardly change. For example, The $\theta$ value of the rate 36Mbps is about 0.77 and $\theta$ value of the rate 24Mbps is about 0.83.


Three algorithms except for SampleRate show
negligible difference, and almost always stick to the best rate (36 Mbps in our case). This contrasts with SampleRate, that shows highly fluctuating patterns: suboptimal rate selections are often made. The reason why SampleRate does not perform well is that actually the channel conditions here correspond to what we referred to as the {\sl Gradual} scenario in the previous subsection. Indeed  4 successive transmissions failures at the best rate often occur, in which case, SampleRate is forced to explore other (suboptimal) rates. Averaged over the 300 seconds, the throughput achieved by KL-U-UCB is 27.12 Mbps, which corresponds to 99.3\% of the throughput under Oracle algorithm (see Table \ref{tab:throughput}). However, SampleRate provides 19 Mbps only -- our algorithm provides 42\% throughput improvement over SampleRate.

% The instant throughput in Fig. \ref{fig:st_result} is calculated by averaging during the last 10 seconds, where the 10 seconds is a length of a time window of samplerate \cite{bicket2005bit}.
% The evaluated algorithms in the Fig. have no time window (except for SampleRate) and our proposed algorithm show negligible differences in instant throughputs.
% They follow the best rate well, and thus their induced throughput is quite similar with the goodput of the best rate.
% However, the bit-rate selected by SampleRate seems to go up and down. This is because


\begin{figure}[htp]
  \centering
  \subfigure[Evolution of $r_k\theta_k$]{%
  \label{fig:st_trace}
  \includegraphics*[width=0.48\columnwidth]{stationary_trace.pdf}} \hspace{-3mm}
 \subfigure[Instantaneous throughput]{
  \label{fig:st_result}
  \includegraphics*[width=0.48\columnwidth]{stationary_result.pdf}}
\caption{Stationary environment -- no mobility}
  \label{fig:st_channel}
\end{figure}


\begin{figure}[htp]
  \centering
  \subfigure[Evolution of $r_k\theta_k$]{%
  \label{fig:nonst_trace}
  \includegraphics*[width=0.48\columnwidth]{nonstationary_trace.pdf}} \hspace{-3mm}
 \subfigure[Instantaneous throughput]{
  \label{fig:nonst_result}
  \includegraphics*[width=0.48\columnwidth]{nonstationary_result.pdf}}
\caption{Non-stationary environment -- mobility}
  \label{fig:nonst_channel}
\end{figure}


\begin{table}[t!]
\begin{center}
\caption{\label{tab:throughput} Average throughput over 300 seconds under several algorithms (Mbps).}
   \begin{tabular}{|c|c|c|c|c|} \hline
      {\bf Scenario} & {\bf Oracle} & {\bf KL-U-UCB} & {\bf KL-R-UCB} & {\bf SampleRate}\\ \hline \hline
      stationary   & 27.29  & 27.12  & 26.85  & 19.32   \\ \hline
      nonstationary  &  23.89  &  22.59 & 22.29  & 16.14  \\ \hline
\end{tabular}
\end{center}
\end{table}

In the case of non-stationary environment, algorithms are
equipped with sliding window of 10 seconds\footnote{SampleRate has a sliding window of 10
  secs, and we use the same value for our algorithms for fair comparison.} to respond to channel variations. In Fig.~\ref{fig:nonst_trace}, we can observe that at the beginning, when the transmitter and receiver are relatively close to each other, the conditions correspond to what we called a {\sl Steep} scenario:  the success transmission probability is high at any rate. Then, as the distance between the transmitter and the receiver increases, the conditions evolve towards those of a {\sl Gradual} and ultimately
{\sl Lossy} scenario.  As shown in Fig.~\ref{fig:nonst_result}, SampleRate initially tracks the best rate quite
well, like our proposed algorithm. However after about 50 seconds, SampleRate deviates from the best rate. This is again due to the fact that consecutive transmission failures even at ``good'' rates occur (Gradual scenario) frequently, in which case, SampleRate decides, by design, not to use these rates. Again in this scenario, KL-U-UCB reveals a tiny gap from Oracle and outperforms SampleRate (the throughput achieved is always at least 20\% greater than that of SampleRate).

% At first, two nodes were close together, and thus the
% channel in Fig. \ref{fig:nonst_trace} starts with a steep condition:
% Every rate has a very high probabilitiy of transmission success. As we
% put some distance between them the channel goes to gradual or lossy
% scenarios. Similar to stationary channel, our proposed algorithms
% correctly chase the best bit-rate but SampleRate does not after 50
% second.  We observed that proposed algorithm bring about 30\% higher
% throughput than SampleRate in average.







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "RA-1"
%%% End:


==> proof2.tex <==
\appendix

\section{Proof of Theorem \ref{th:lower_dep}}

We derive here the regret lower bounds for the MAB problem $(P_U)$. To this aim, we apply the techniques used by Graves and Lai \cite{graves1997} to investigate efficient adaptive decision rules in controlled Markov chains. We recall here their general framework. Consider a controlled Markov chain $(X_t)_{t\ge 0}$ on a finite state space ${\cal S}$ with a control set $U$. The transition probabilities given control $u\in U$ are parametrized by $\theta$ taking values in a compact metric space $\Theta$: the probability to move from state $x$ to state $y$ given the control $u$ and the parameter $\theta$ is $p(x,y;u,\theta)$. The parameter $\theta$ is not known. The decision maker is provided with a finite set of stationary control laws $G=\{g_1,\ldots,g_K\}$ where each control law $g_j$ is a mapping from ${\cal S}$ to $U$: when control law $g_j$ is applied in state $x$, the applied control is $u=g_j(x)$. It is assumed that if the decision maker always selects the same control law $g$ the Markov chain is then irreducible with stationary distribution $\pi_\theta^g$. Now the reward obtained when applying control $u$ in state $x$ is denoted by $r(x,u)$, so that the expected reward achieved under control law $g$ is: $\mu_\theta(g)=\sum_xr(x,g(x))\pi_\theta^g(x)$. There is an optimal control law given $\theta$ whose expected reward is denoted $\mu_\theta^{\star}\in \arg\max_{g\in G} \mu_\theta(g)$. Now the objective of the decision maker is to sequentially control laws so as to maximize the expected reward up to a given time horizon $T$. As for MAB problems, the performance of a decision scheme can be quantified through the notion of regret which compares the expected reward to that obtained by always applying the optimal control law.

We now apply the above framework to our MAB problem. For $(P_U)$, the parameter $\theta$ takes values in ${\cal T}\cap {\cal U}$. The Markov chain has values in ${\cal S}=\{0,r_1,\ldots,r_K\}$. The set of control laws is $G=\{1,\ldots,K\}$. These laws are constant, in the sense that the control applied by control law $k$ does not depend on the state of the Markov chain, and corresponds to selecting rate $r_k$. The transition probabilities are given as follows: for all $x,y\in {\cal S}$, 
$$
p(x,y;k,\theta)=p(y;k,\theta)=\left\{
\begin{array}{ll}
\theta_k, & \hbox{ if }y=r_k,\\
1-\theta_k, & \hbox{ if }y=0.
\end{array}\right.
$$
Finally, the reward $r(x,k)$ does not depend on the state and is equal to $r_k\theta_k$, which is also the expected reward obtained by always using control law $k$. 

We now fix $\theta\in {\cal T}\cap {\cal U}$. Define $I^k(\theta,\lambda)=I(\theta_k,\lambda_k)$ for any $k$. Further define the set $B(\theta)$ consisting of all {\it bad} parameters $\lambda\in {\cal T}\cap{\cal U}$ such that $k^{\star}$ is not optimal under parameter $\lambda$, but which are statistically {\it indistinguishable} from $\theta$:
$$
B(\theta)=\{ \lambda \in {\cal T}\cap {\cal U} : \lambda_{k^{\star}} = \theta_{k^{\star}} \textrm{ and }  \max_k  r_k\lambda_k > r_{k^{\star}}\lambda_{k^{\star}} \},
$$
$B(\theta)$ can be written as the union of sets $B_k(\theta)$, $k=1,\ldots,K$ defined as:
$$
B_k(\theta)=\{ \lambda \in B(\theta) :  r_k\lambda_k > r_{k^{\star}}\lambda_{k^{\star}} \}.
$$
Note that $B_k(\theta)=\emptyset$ if $r_k<r_{k^\star}\theta_{k^\star}$. Define $P=\{k: r_k\ge r_{k^\star}\theta_{k^\star}\}$. Observe that there exist $k_0$ and $k_1$ such that $k_0\le k^\star\le k_1$ and $P=\{k_0,\ldots,k_1\}$. Further define $P'=P\setminus\{k^\star\}$.

By applying Theorem 1 in \cite{graves1997}, we know that $c(\theta)$ is the minimal value of the following LP:
\begin {eqnarray}
\textrm{min }  & \sum_k c_k(r_{k^{\star}}\theta_{k^{\star}} - r_k\theta_k) \\
\textrm{s.t. } & \inf_{\lambda \in B_k(\theta)} \sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda) \geq 1, \quad \forall k \in P' \label{eq:con1}\\
& c_k \geq 0, \quad \forall k .
\end {eqnarray}

Next we show that the constraints (\ref{eq:con1}) on the $c_k$'s are equivalent to:
\begin{equation}\label{eq:con2}
\min_{k\in N(k^\star)} c_{k}I(\theta_k,{r_{k^\star}\theta_{k^\star}\over r_k}) \ge 1.
\end{equation}
To this aim, let $k\in P'$. Without loss of generality assume that $k>k^\star$. We prove that:
\begin{equation}\label{eq:inf}
\inf_{\lambda \in B_k(\theta)} \sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda) = \sum_{l=k^\star+1}^k c_lI(\theta_l,{r_{k^\star}\theta_{k^\star}\over r_l}).
\end{equation}
This is simply due to the following two observations:
\begin{itemize}
\item for all $\lambda\in B_k(\theta)$, we have $\lambda_{k^\star}r_{k^\star}= \theta_{k^\star}r_{k^\star}$ and $\lambda_{k}r_{k}> \lambda_{k^\star}r_{k^\star}$, which using the unimodality of $\lambda$, implies that for any $l\in \{k^\star,\ldots,k\}$, $\lambda_{l}r_l\ge \theta_{k^\star}r_{k^\star}$. Hence:
$$
\sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda) \ge \sum_{l=k^\star+1}^k c_lI(\theta_l,{r_{k^\star}\theta_{k^\star}\over r_l}).
$$
\item For $\epsilon >0$, define $\lambda_\epsilon$ as follows: for all $l\in \{k^\star,\ldots,k\}$, $\lambda_l = (1+(l-k^\star)\epsilon) {r_{k^\star}\theta_{k^\star}\over r_l}$, and for all $l\notin \{k^\star,\ldots,k\}$, $\lambda_l=\theta_l$. By construction, $\lambda_\epsilon\in B_k(\theta)$, and 
$$
\lim_{\epsilon\to 0} \sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda_\epsilon) = \sum_{l=k^\star+1}^k c_lI(\theta_l,{r_{k^\star}\theta_{k^\star}\over r_l}).
$$
\end{itemize}

From (\ref{eq:inf}), we deduce that constraints (\ref{eq:con1}) are equivalent to (\ref{eq:con2}) (indeed, only the constraints related to $k\in N(k^\star)$ are really active, and for $k\in N(k^\star)$, (\ref{eq:con1}) is equivalent to $c_{k}I(\theta_k,{r_{k^\star}\theta_{k^\star}\over r_k}) \ge 1$). With the constraints (\ref{eq:con2}), the optimization problem becomes straightforward to solve, and its solution yields: 
$$
c(\theta) = \sum_{k\in N(k^\star)} {r_{k^{\star}}\theta_{k^{\star}} - r_k\theta_k) \over I(\theta_k,{r_{k^\star}\theta_{k^\star}\over r_k})}.
$$
\ep

\section{Proof of Theorem \ref{th:lower_indep}}

The proof of Theorem \ref{th:lower_indep} is similar to that of Theorem \ref{th:lower_dep}. The only difference is that in absence of correlations and unimodality, we can only assume that the parameter $\theta$ takes values in $[0,1]^K$. 

In what follows, we fix $\theta\in [0,1]^K$, and denote by $k^{\star}$ the index of the optimal rate. The sets $B(\theta)$ and $B_k(\theta)$ are now defined as:
$$
B(\theta)=\{ \lambda \in [0,1]^K : \lambda_{k^{\star}} = \theta_{k^{\star}} \textrm{ and }  \max_k  r_k\lambda_k > r_{k^{\star}}\lambda_{k^{\star}} \}.
$$
$$
B_k(\theta)=\{ \lambda \in B(\theta) :  r_k\lambda_k > r_{k^{\star}}\lambda_{k^{\star}} \}.
$$
By applying Theorem 1 in \cite{graves1997}, we know that $c'(\theta)$ is the minimal value of the following optimization problem:
\begin {eqnarray*}
\begin {array}{ll}
\textrm{min }  & \sum_k c_k(r_{k^{\star}}\theta_{k^{\star}} - r_k\theta_k) \\
\textrm{s.t. } & \inf_{\lambda \in B_k(\theta)} \sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda) \geq 1, \quad \forall k \neq k^{\star} \\
& c_k \geq 0, \quad \forall k .
\end{array}
\end {eqnarray*}
We now solve :
$
\inf_{\lambda \in B_k(\theta)} \sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda).
$  
Remark that for $k<k_0$, $B_k(\theta)=\emptyset$, because $r_{k^{\star}}\theta_{k^{\star}}>r_k$ for $k<k_0$. Let $k\ge k_0$. For any fixed $\theta$ and all $l$,
$$
I^l(\theta,\lambda) = \theta_l \log \frac{\theta_l}{\lambda_l} + (1-\theta_l) \log \frac{1-\theta_l}{1-\lambda_l}
$$
is a convex in $\lambda_l$ and it achieves its minimum (equal to $0$) at $\lambda_l = \theta_l$.
Hence, we can choose $\lambda_l = \theta_l$, for all $l \neq k$. Since $\lambda \in B_k(\theta)$, we must have $\lambda_k > \frac{r_{k^{\star}}\theta_{k^{\star}}}{r_k} $. Hence from the convexity of $I(\theta_k,\lambda_k)$ in $\lambda_k$, we get:
$$
\inf_{\lambda_k:\lambda_k > \frac{r_{k^{\star}}\theta_{k^{\star}}}{r_k}}I(\theta_k,\lambda_k)=I(\theta_k,\frac{r_{k^{\star}}\theta_{k^{\star}}}{r_k}).
$$
We deduce that
$
\inf_{\lambda \in B_k(\theta)} \sum_{l \neq k^{\star}} c_lI^{l}(\theta,\lambda)  =  c_kI(\theta_k, \frac{r_{k^{\star}}\theta_{k^{\star}}}{r_k}),
$
where the infimum is reached for $\lambda=(\theta_1,\dots,\theta_{k-1}, \frac{r_{k^{\star}}\theta_{k^{\star}}}{r_k}, \theta_{k+1}, \dots, \theta_K)$. Finally we obtain that:
$$
c'(\theta) =\sum_{k=k_0, k\neq k^{\star}}^K {r_{k^{\star}}\theta_{k^{\star}}-r_k\theta_k\over I(\theta_k, \frac{r_{k^{\star}}\theta_{k^{\star}}}{r_k})}.
$$


\section{Proof of Theorem \ref{th:KL-UCB-R2}} 

{\bf Notations.} Throughout the proofs, by a slight abuse of notation, we omit the floor/ceiling functions when it does not create ambiguity.	Consider a suboptimal rate $k \neq k^\star$. If $k$ has only one neighbor, we denote it by ${k}_2$ and we must have $\theta_k r_k < \theta_{{k}_2} r_{{k}_2}$ since $k$ is suboptimal. Otherwise we denote by ${k}_1$ and ${k}_2$ the neighbors of $k$ with $\theta_{{k}_1} r_{{k}_1} <  \theta_k r_k < \theta_{{k}_2} r_{{k}_2}$.

Define the difference between the average reward of $k$ and $k^\prime$ : $\Delta_{k,k^\prime} = | \theta_{k^\prime} r_{k^\prime} - \theta_{k} r_{k}|  > 0$. We use the notation: 
\eq{
\hat\mu_{k,s} = \frac{1}{s} \sum_{i=1}^s r_k X_k(i).
}
and:
\eq{
t_{k,k^\prime}(n) = \sum_{n^\prime=1}^n \indic \{ L(n) = k, k(n) = k^\prime \}.
}
$t_{k,k^\prime}(n)$ is the number of times that $k^\prime$ is when $k$ is the leader.

\noindent
{\bf Proof.} Let $T>0$, and $\pi$=KL-U-UCB. The regret $R^\pi(T)$ of KL-U-UCB up to time $T$ is:
$$
R^{\pi}(T) = \sum_{k\neq k^\star} (r_{k^\star} \theta_{k^\star} - r_k \theta_k  ) \EE[ \sum_{n=1}^T   \indic\{ k(n)=k\} ].
$$
We use the following decomposition:
$$
\indic\{ k(n)=k\}=\indic\{L(n)=k^\star,k(n)=k\} +\indic\{L(n)\neq k^\star,k(n)=k\}.
$$
Now 
\begin{align*}
\sum_{k\neq k^\star}   (r_{k^\star} \theta_{k^\star} - r_k \theta_k  ) & \EE[ \sum_{n=1}^T   \indic\{ L(n)\neq k^\star, k(n)=k\} ]\\
& \le r_{k^\star}\sum_{k\neq k^\star}\EE[ \sum_{n=1}^T   \indic\{ L(n)\neq k^\star,k(n)=k\} ] \\
&\le r_{k^\star}\sum_{k\neq k^\star}\EE[ l_k(T)].
\end{align*}
Observing that when $L(n)=k^\star$, the algorithm selects a decision $k\in N(k^\star)$, we deduce that: 
\begin{align*}
R^{\pi}(T) \leq  r_{k^\star} \sum_{k \neq k^\star } \EE[  l_k(T) ]   +  \sum_{k \in N(k^\star)} (r_{k^\star} \theta_{k^\star} - r_k \theta_k  ) \EE[ \sum_{n=1}^T   \indic \{ L(n) = k^\star , k(n) = k \} ] 
\end{align*}

Then we analyze the two terms in the r.h.s. in the above inequality. The first term corresponds to the average number of times where $k^\star$ is not the leader, while the second term represents the accumulated regret when the leader is $k^\star$. The following result states that the first term is $O(\log(\log(T)))$:

\begin{theorem} \label{lemma:l1bound}
For $k \neq k^\star$, $ \EE[ l_k(T) ] = O(\log(\log(T)))$.
\end{theorem}

From the above theorem, we conclude that the leader is $k^\star$ except for a negligible number of instants (in expectation). When $k^\star$ is the leader, KL-U-UCB behaves as KL-UCB restricted to the set $N(k^\star)$ of possible decisions. Following the same analysis as in \cite{garivier2011} (the analysis of KL-UCB), we can show that for all $\epsilon > 0$ there are constants $C_1 \leq 7$ , $C_2(\epsilon)$ and $\beta(\epsilon) > 0$ such that:
\begin{align}
\EE[ \sum_{n=1}^T  \indic \{L(n) = k^\star , k(n) = k \} ]  & \leq  \EE[ \sum_{n=1}^T  \indic \{  b_{k}(n) \geq   b_{k^\star}(n) \} ]    \sk 
& \leq (1 + \epsilon) \frac{\log (T)}{I(\theta_k, \frac{r_{k^\star} \theta_{k^\star}}{r_k})}   + C_1 \log(\log(T)) + \frac{C_2(\epsilon)}{T^{\beta(\epsilon)}}.
\end{align}
Combining the above bound with Theorem \ref{lemma:l1bound}, we get:
\begin{align}\label{ref:regretlead2}
R^{\pi}(T) & \leq   (1 + \epsilon) c(\theta) \log (T) +  O( \log(\log(T)) ),
\end{align}
which concludes the proof of Theorem \ref{th:KL-UCB-R2}.
\ep

It remains to show that Theorem \ref{lemma:l1bound} holds, which is done in the next section.


\section{Proof of Theorem \ref{lemma:l1bound}}

The proof of Theorem \ref{lemma:l1bound} is technical, and requires a few preliminary results presented in \ref{sec:conc}, \ref{sec:dev}, and \ref{sec:kl}. The theorem itself is proved in \ref{sec:pro}.

\subsection{Hoeffding's inequality}\label{sec:conc}
 
 We recall the Hoeffding's inequality which is used throughout the proofs.

\begin{lemma}\label{lem:hoeffding}[Hoeffding's inequality]
Let $\{ Z_t \}_{1 \leq t \leq n}$ be a sequence of independent random variables with, for any $t$, $ Z_t \in [a_t,b_t]$ almost surely. We have, for any $\delta >0$:
$$ 
\PP\bigg[   \big| \sum_{t=1}^n (Z_t - \EE[Z_t]) \big| \geq \delta  \bigg] \leq 2 \exp\left( -\frac{2 \delta^2}{\sum_{t=1}^n (b_t - a_t)^2} \right).
$$
\end{lemma} 
 
%\begin{lemma}\label{lem:sanov}[Sanov's theorem]
%Let $\{ Z_t \}_{1 \leq t \leq n}$ be a sequence of i.i.d Bernoulli random variables with mean $q$, and ${\cal Q} \subset [0,1]$, then:
%$$
%\PP \Lb \Lp \frac{1}{n} \sum_{t=1}^n Z_t \Rp \in {\cal Q} \Rb \leq (n + 1)^2 2^{ - n \inf_{p \in {\cal Q} }I(p,q)}.
%$$
%\end{lemma} 
 
  \subsection{Deviation bounds}\label{sec:dev} 

The following two lemmas are used repeatedly in the proof of Theorem~\ref{lemma:l1bound}. They are corollaries of Hoeffding's inequality and allow us to show that certain families of events happen only rarely (in expectation). 
 
Lemma~\ref{lem:deviation} states that if a set of instants $\Lambda$ can be decomposed into a family of subsets $(\Lambda(s))_{s\ge 1}$ of finite sizes and where $k$ is tried sufficiently many times ($t_k(n) \geq \epsilon s$ , $n \in \Lambda(s)$), then the expected number of instants in $\Lambda$ at which the average reward of $k$ is badly estimated is finite.
 
\begin{lemma}\label{lem:deviation}
Let $k\in\{ 1,\ldots,K\}$, and $\epsilon >0$. Let $\Lambda \subset \NN$ be a (random) set of instants. Assume that there exists a sequence of (random) sets $(\Lambda(s))_{s\ge 1}$ such that (i) $\Lambda \subset \cup_{s \geq 1} \Lambda(s)$, and (ii) for all $s\ge 1$ and all $n\in \Lambda(s)$, $t_k(n)\ge \epsilon s$. Further assume that there exists a deterministic function $\overline{\Lambda}$ such that for all $s$ we have $|\Lambda(s)| \leq \overline{\Lambda}(s)$ almost surely. 
Then for all $\delta > 0$: 
\begin{equation}\label{eq:ineq1}
\EE[ \sum_{n \geq 1} \indic\{ n \in \Lambda , | \hat\mu_k(n) - \theta_k r_k  | > \delta \} ] \leq \frac{2}{1 - \exp( -\frac{ 2 \delta^2}{r_k^2})} \sum_{s \geq 1} \overline{\Lambda}(s) \exp \Lp - \frac{ 2 s \epsilon  \delta^2}{r_k^2} \Rp.
\end{equation}
In particular, if there exists a constant $\overline{\Lambda}$ such that $\overline{\Lambda}(s) \leq \overline{\Lambda}$ for all $s$:
\begin{equation}\label{eq:ineq2}
\EE[ \sum_{n \geq 1} \indic\{ n \in \Lambda , | \hat\mu_k(n) - \theta_k r_k  | > \delta \} ] \leq \frac{ 2 \overline{\Lambda}}{( 1 - \exp( -\frac{ 2 \delta^2}{r_k^2}))( 1 - \exp( -\frac{ 2 \epsilon \delta^2}{r_k^2}))}.
\end{equation}
More generally if $s \mapsto \overline{\Lambda}(s)$ grows at most polynomially:
\begin{equation}\label{eq:ineq3}
\EE[ \sum_{n \geq 1} \indic\{ n \in \Lambda , | \hat\mu_k(n) - \theta_k r_k  | > \delta \} ] < +\infty.
\end{equation}
\end{lemma}
\bp
Since $\Lambda \subset \cup_{s \geq 1} \Lambda(s)$, we have:
\begin{align*}
\sum_{n \geq 1} \indic\{ n \in \Lambda , | \hat\mu_k(n) - \theta_k r_k  | > \delta \} & \leq \sum_{n \geq 1} \sum_{s \geq 1} \indic \{ n \in \Lambda(s) , | \hat\mu_k(n) - \theta_k r_k  | > \delta , t_k(n) \geq \epsilon s \} \\
 	& \leq \sum_{n \geq 1} \sum_{s \geq 1} \indic \{ n \in \Lambda(s) \} \indic \{  \sup_{s^\prime \geq s \epsilon}   | \hat\mu_{k,s^\prime} - \theta_k r_k  | > \delta \} \\
 	& \leq \sum_{s \geq 1} \overline{\Lambda}(s) \indic\{  \sup_{s^\prime \geq s \epsilon}   | \hat\mu_{k,s^\prime} - \theta_k r_k  | > \delta \},
\end{align*}
where the last inequality is due to the fact that $\sum_{n \geq 1}  \indic \{ n \in \Lambda(s) \} \leq  \overline{\Lambda}(s)$ almost surely. Applying the Hoeffding's inequality and union bound, we get:
\begin{align*}
\PP[ \sup_{s^\prime \geq s \epsilon}   | \hat\mu_{k,s^\prime} - \theta_k r_k  | > \delta  ] &\leq \sum_{s^\prime \geq s \epsilon} \PP[  | \hat\mu_{k,s^\prime} - \theta_k r_k  | > \delta ] \\
& \leq \sum_{s^\prime \geq s \epsilon} 2 \exp(  - \frac{ 2 s^\prime  \delta^2}{r_k^2}    ) \\
& \leq \frac{2 \exp(  - \frac{ 2 s \epsilon  \delta^2}{r_k^2})}{1 - \exp( -\frac{ 2 \delta^2}{r_k^2})}     ,
\end{align*}
Summing over $s$, we obtain (\ref{eq:ineq1}):
$$
\EE[ \sum_{n \geq 1} \indic \{ n \in \Lambda , | \hat\mu_k(n) - \theta_k r_k  | > \delta \} ]   \leq  \frac{2}{1 - \exp( -\frac{ 2 \delta^2}{r_k^2})} 
	\sum_{s \geq 1} \overline{\Lambda}(s) \exp \Lp - \frac{ 2 s \epsilon  \delta^2}{r_k^2} \Rp  .
$$
(\ref{eq:ineq2}) and (\ref{eq:ineq3}) are direct applications of (\ref{eq:ineq1}). \ep


% The second inequality is obtained by setting $\overline{\Lambda}(s) = \overline{\Lambda}$:
 %\eq{
 %\EE[ \sum_{n \geq 1} \indic \{ n \in \Lambda , | \hat\mu_k(n) - \theta_k r_k  | > \delta \} ]  \leq \frac{2  \overline{\Lambda}}{( 1 - \exp( -\frac{ 2 \delta^2}{r_k^2}))( 1 - \exp( -\frac{ 2 \epsilon \delta^2}{r_k^2}))} . 
 %}
 %The third inequality is proven similarly.

A useful corollary of lemma~\ref{lem:deviation} is obtained by choosing $\delta = \Delta_{k,k^\prime}/2$: 
%if for a given family of events, $k$ and $k^\prime$ are both tried frequently enough, then the one which has a smaller mean reward is the leader only finitely many times.
 
\begin{lemma}\label{cor:deviation}
Let $k, k'\in\{ 1,\ldots,K\}$ with $k\neq k'$ and $r_k \theta_k \leq r_{k^\prime} \theta_{k^\prime}$ and $\epsilon >0$. Let $\Lambda \subset \NN$ be a (random) set of instants. Assume that there exists a sequence of (random) sets $(\Lambda(s))_{s\ge 1}$ such that (i) $\Lambda \subset \cup_{s \geq 1} \Lambda(s)$, and (ii) for all $s\ge 1$ and all $n\in \Lambda(s)$, $t_k(n)\ge \epsilon s$ and $t_{k'}(n)\ge \epsilon s$. Further assume that there exists a deterministic function $\overline{\Lambda}$ such that for all $s$ we have $|\Lambda(s)| \leq \overline{\Lambda}(s)$ almost surely. 
Then, if $s \mapsto \overline{\Lambda}(s)$ grows at most polynomially, 
\begin{equation}\label{eq:ineq4}
\EE[ \sum_{n \geq 1} \indic \{ n \in \Lambda ,  \hat\mu_k(n) \geq \hat\mu_{k^\prime}(n) \} ] < +\infty. 
\end{equation}
\end{lemma}

\subsection{KL divergence }\label{sec:kl} 
 
We present results related to the KL divergence that will be instrumental when manipulating indexes $b_k(n)$. Lemma~\ref{lem:pinsker} gives an upper and a lower bound for the KL divergence. The lower bound is Pinsker's inequality. The upper bound is due to the fact that $I(p,q)$ is convex in its second argument.
\begin{lemma}\label{lem:pinsker}[Pinsker's inequality]
For all $p,q \in [0,1]^2$, $p \leq q$:
\eq{
 2 (p - q)^2 \leq I(p,q) \leq \frac{ (p-q)^2 }{q(1-q)}.
 }
 Also: 
 \eq{\label{eq:pinkser_equiv}
  I(p,q)  \sim  \frac{ (p-q)^2 }{p(1-p)}.
  }
 when $q \to p^+$.
\end{lemma}
\bp
	The lower bound is Pinsker's inequality. 
	We consider the upper bound. The derivative of the KL divergence is:
	\eq{
	\frac{\partial I}{\partial q}\Lp p,q \Rp = \frac{q-p}{q(1-q)}.
	}
	Since $q \mapsto \frac{\partial I}{\partial q}(p,q)$ is increasing, the fundamental theorem of calculus gives the announced result:
	\eq{
	I(p,q) \leq \int_{p}^{q} \frac{\partial I}{\partial u} \Lp p,u \Rp du \leq \frac{(p-q)^2}{q(1-q)}. 
	}
	The equivalence comes from a Taylor development of $q \to I(p,q)$ at $p$, since: 
	\eq{
	\frac{\partial I}{\partial q}(p,q) |_{q=p} = 0, \sk
	\frac{\partial^2 I}{\partial q^2}(p,q) |_{q=p} = \frac{1}{q(1-q)}.
	}
\ep
	
%\begin{lemma}\label{lem:kldivleader}
%Let $k, k'\in\{ 1,\ldots,K\}$ with $k\neq k'$, and $n\in\mathbb{N}$. Assume that $L(n)=k$. Then:
%\begin{itemize}
%\item[(i)] If $r_{k} > r_{k^\prime}$ and $t_k(n) \leq  t_{k^\prime}(n)$ then $b_k(n) > b_{k^\prime}(n)$.
%\item[(ii)] Let us fix $\delta > 0$ and $\epsilon > 0$ small enough and $\overline{\mu} \in (0,r_{k^\prime})$. Then there exists $s_0$ such that if $t_{k}(n)  \leq \epsilon l_k(n)$ ,  $t_{k^\prime}(n) \geq l_k(n)/2$ , $| \hat\mu_{k^\prime}(n)- \overline{\mu}| < \delta$ , and $l_k(n) \geq s_0$ then $b_k(n) > b_{k^\prime}(n)$
%\end{itemize}
%\end{lemma}
%	
%\bp
%(i) Let $q \in [\hat\mu_{k}(n),r_{k}]$. We have:
%\begin{align*}
%t_{k}(n) I \Lp \frac{\hat\mu_{k}(n) }{r_{k}} ,   \frac{ q }{r_{k}} \Rp
%& \leq t_{k^\prime}(n) I \Lp \frac{\hat\mu_{k^\prime}(n) }{r_{k}} ,   \frac{ q }{r_{k}} \Rp \\ 
%& \leq t_{k^\prime}(n) I \Lp \frac{\hat\mu_{k^\prime}(n)}{r_{k^\prime}} ,   \frac{q}{r_{k^\prime}} \Rp,
%\end{align*}
%where the second inequality is obtained observing that $\mu \to I(p\mu,q\mu)$ is increasing on $[0,1]$ for $p < q$. We conclude that $b_k(n)<b_{k'}(n)$.
%	
%(ii) Define $s = l_k(n)$. Using Pinsker's inequality we have that:
%	\eq{
%		b_{k^\prime}(n) \leq \hat\mu_{k^\prime}(n) + r_{k^\prime} \sqrt{ \frac{ \log(s) + c \log ( \log (s) )  }{2 t_{k^\prime}(n)} }  \leq \hat\mu_{k^\prime}(n) + r_{k^\prime} \sqrt{ \frac{ \log(s) + c \log ( \log (s) )  }{s} }.
%	}
%	We then have the inequality:
%	\al{ \label{eq:lem:kldiv}
%		t_{k}(n) I \Lp \frac{\hat\mu_{k}(n) }{r_{k}} ,   \frac{b_{k^\prime}(n) }{r_{k}}   \Rp & \leq \epsilon s I \Lp \frac{\hat\mu_{k^\prime}(n) }{r_{k}} ,\frac{b_{k^\prime}(n) }{r_{k}} \Rp \\
%		& \leq \epsilon s I \Lp \frac{\hat\mu_{k^\prime}(n) }{r_{k}} ,\frac{\hat\mu_{k^\prime}(n) }{r_{k}} +   \frac{r_{k^\prime}}{r_k} \sqrt{ \frac{ \log(s) + c \log ( \log (s) )  }{s} } \Rp \\
%		& \leq \sup_{ | \mu - \overline{\mu}| < \delta} \epsilon s I \Lp \frac{\mu}{r_{k}} ,\frac{\mu}{r_{k}} +  \frac{r_{k^\prime}}{r_k} \sqrt{ \frac{ \log(s) + c \log ( \log (s) )  }{s} } \Rp  \\
%		& \sim_{s \to +\infty} \Lp \log(s) + c \log ( \log (s) ) \Rp \frac{2 \epsilon r_{k^\prime}^2 }{r_{k}^2} + O(\delta) \\
%		& <  \log(s) + c \log ( \log (s) ),
%	}
%	for $\delta$ and $\epsilon$ small enough, using the differentiability of the KL divergence. So there exists $s_0$ such that if $s \geq s_0$ the l.h.s of~\eqref{eq:lem:kldiv} is strictly smaller than $\log(s) + c \log ( \log (s) )$ and hence $b_{k}(n) > b_{k^\prime}(n)$ proving the result.
%	
%	\ep

Lemma~\ref{lem:deviation_result} is straightforward from \cite{garivier2011}[Theorem 10]. It should be observed that this result is not a direct application of Sanov's theorem; Lemma \ref{lem:deviation_result} provides sharper bounds in certain cases.	

\begin{lemma}\label{lem:deviation_result}
For $1 \leq t_k(n)  \leq \tau$ and $\delta > 0$, if $\{ X_k(i) \}_{1 \leq i \leq \tau}$ are i.i.d Bernoulli random variables with parameter $\theta_k$, we have that:
$$
\PP \Lb t_k(n) I \Lp  \frac{1}{t_k(n)} \sum_{i=1}^{t_k(n)} X_k(i) , \theta_k \Rp \geq \delta  \Rb \leq 2 e \ceil{\delta \log(\tau) }\exp(-\delta).	
$$
\end{lemma}
	
\subsection{Proof of Theorem~\ref{lemma:l1bound} }\label{sec:pro} 

Let $k$ be the index of a suboptimal rate under. Let  $\delta > 0$, $\epsilon > 0$ small enough (we provide a more precise definition later on). To derive an upper bound of $\mathbb{E}[l_k(T)]$, we decompose the set of times where $k$ is the leader into the following sets:
$$
\{n \leq T: L(n)=k\}\subset A_\epsilon\cup B_{\epsilon}^T,
$$
where
\begin{align*}
A_{\epsilon} & =  \{ n:	L(n) = k ,  t_{k_2}(n) \geq \epsilon l_k(n) \}\\
B_{\epsilon}^T &= \{  n \leq T: L(n) = k , t_{k_2}(n) \leq \epsilon l_k(n)\}.
\end{align*}
Hence we have:
\begin{equation*}
 \mathbb{E}[l_k(T)] \leq \mathbb{E}\big[ |A_{\epsilon}| + |B_{\epsilon}^T| \big],
\end{equation*}	
Next we provide upper bounds of $\mathbb{E}[ |A_{\epsilon}|]$ and $\mathbb{E}[ |B_{\epsilon}^T |]$. 

\medskip
\noindent
\underline{Bound on $\mathbb{E} |A_\epsilon|$.} Let $n \in A_{\epsilon}$ and assume that $l_k(n)=s$. By design of the algorithm, $t_{k}(n) \geq s/3$. Also  $t_{k_2}(n) \geq \epsilon l_k(n) = \epsilon s$. We apply Lemma~\ref{cor:deviation} with $\Lambda(s) = \{ n  \in A_{\epsilon} , l_k(n) = s  \}$, $\Lambda =\cup_{s\ge 1}\Lambda(s)$. Of course, for any $s$, $|\Lambda(s)| \leq 1$. We have: $A_\epsilon =\{n\in \Lambda:\hat{\mu}_k(n)\ge \hat{\mu}_{k_2}(n)\}$, since when $n\in A_\epsilon$, $k$ is the leader. Lemma~\ref{cor:deviation} can be applied with $k'=k_2$. We get: $\EE| A_{\epsilon}|  < \infty$.

\medskip
\noindent
\underline{Bound on $\mathbb{E} |B_{\epsilon}^T|$.} We introduce the following sets
\begin{itemize}
\item[] $C_\delta = C_{\delta,1}\cup C_{2}$ is the set of instants at which the average reward of the leader $k$ is badly estimated:
\begin{align*}
C_{\delta,1} &= \{  n:  L(n) = k ,  | \hat{\mu}_k(n) - \theta_k r_k | > \delta  \}\\
C_{2} &= \{  n: L(n) = k , k_2 \notin  M(k, \hat{\mu}_k(n))  \};
\end{align*}
\item[] $D_{\delta} = D_{\delta,k}\cup D_{\delta,k_1}$ where $D_{\delta,k'}=\{ n: L(n) = k , k(n) = k^\prime ,  | \hat{\mu}_{k^\prime}(n) - \theta_{k^\prime} r_{k^\prime} | > \delta \}$  is the set of instants at which $k$ is the leader, $k^\prime$ is selected and the average reward of $k^\prime$ is badly estimated.
\item[] $E^T = \{ n \leq T: L(n) = k , b_{k_2}(n) \leq \theta_{k_2} r_{k_2} \}$, is the set of instants at which $k$ is the leader, and the upper confidence index $b_{k_2}(n)$ underestimates the average reward $\theta_{k_2} r_{k_2}$.
\end{itemize}
We first prove that $|B_{\epsilon}^T| \leq 12(|C_\delta| + |D_{\delta}| + |E^T|) + O(1)$ as $T$ grows large, and then provide upper bounds on $\mathbb{E}|C_\delta|$, $\mathbb{E}|D_\delta|$, and $\mathbb{E}|E^T|$. Namely, if $k_2$ has not been tried many times, it either means that the index $b_{k_2}(n)$ underestimates the mean reward $\theta_{k_2} r_{k_2}$, or that the average reward of one of the selected arms (or the leader) deviates from its mean reward.

	Consider $n \in B_{\epsilon}^T$. When $k$ is the leader, only $\{ k_1, k , k_2 \}$ can be selected:
\eq{
l_k(n) = t_{k,k_1}(n) + t_{k,k}(n) + t_{k,k_2}(n) \leq   t_{k,k_1}(n) + t_{k,k}(n) + \epsilon l_k(n).
}
So $t_{k,k_1}(n) + t_{k,k}(n) \geq (1 - \epsilon) l_k(n)$. Consider $\epsilon < 1/6$, we must have that either (a) $t_{k,k_1}(n) \geq l_k(n)/3$ or (b) $t_{k,k}(n) \geq l_k(n)/2 + 1$, otherwise $t_{k,k_1}(n) + t_{k,k}(n) \geq (1 - \epsilon) l_k(n)$ does not hold.

	(a) Assume that $t_{k,k_1}(n) \geq l_k(n)/3$.  Since $t_{k,k_1}(n)$ is only incremented when $k_1$ is selected and $k$ is the leader, and since $n \mapsto l_k(n)$ is increasing, there exists a unique $\phi(n) < n$ such that $L(\phi(n)) = k$, $k(\phi(n)) = k_1$, $t_{k,k_1}(\phi(n)) = \floor{l_k(n)/6}$. $\phi(n)$ is indeed unique because $t_{k,k_1}(\phi(n))$ is incremented at time $\phi(n)$.
	
	We are going to prove that for $l_k(n) \geq l_0$ large enough and $\delta$ small enough we must have $\phi(n) \in C_\delta \cup D_{\delta} \cup E^T$. Assume that $\phi(n) \notin C_\delta \cup D_{\delta} \cup E^T$. Then $b_{k_2}(\phi(n)) \geq \theta_{k_2} r_{k_2}$ and $\hat\mu_{k_1}(\phi(n)) \leq \theta_{k_1} r_{k_1} + \delta$. Using Pinsker's inequality and the fact that $t_{k_1}(\phi(n)) \geq t_{k,k_1}(\phi(n))$:
	\al{
		b_{k_1}(\phi(n)) & \leq \hat\mu_{k_1}(\phi(n)) + \sqrt{\frac{ \log(l_k(\phi(n))) + c \log(\log(l_k(\phi(n))))   }{ 2 t_{k_1}(\phi(n)) }   } \sk
		 & \leq   \theta_{k_1} r_{k_1} + \delta + \sqrt{\frac{ \log(l_k(n)) + c \log(\log(l_k(n)))}{ 2 \floor{ l_k(n)/6}}} \sk
		 & \leq   \theta_{k_1} r_{k_1} + 2 \delta < \theta_{k_2} r_{k_2} \leq b_{k_2}(\phi(n)).
	}
	$l_k(n) \geq l_0$ large enough and $\delta$ small enough. Namely, $\delta < (\theta_{k_2} r_{k_2} - \theta_{k} r_{k})/2$ and $l_0$ such that  $\sqrt{ (\log(l_0) + c \log(\log(l_0)))/ 2 \floor{l_0/6}}  \leq \delta$.

	 Therefore $\phi(n) \in C_{\delta} \cup D_{\delta} \cup E^T$, otherwise we cannot have $k(\phi(n)) = k_1$. Indeed $\phi(n) \notin C_{\delta} \cup D_{\delta} \cup E^T$ implies $b_{k_1}(\phi(n)) < b_{k_2}(\phi(n))$, and $k_2 \in  M(k, \hat{\mu}_k(n))$ which is incompatible with $k(\phi(n)) = k_1$.
	
	(b) Assume that $t_{k,k}(n) \geq l_k(n)/2 + 1 = l_k(n)/3 + l_k(n)/6 + 1$. There are at least $l_k(n)/6 + 1$ instants $\tilde{n}$ such that $l_{k}(\tilde{n}) - 1$ is not a multiple of $3$, $L(\tilde{n}) = k$ and $k(\tilde{n}) = k$. By the same reasoning as in (a) there exists a unique $\phi(n) < n$ such that $L(\phi(n)) = k$, $k(\phi(n)) = k$ , $t_{k,k}(\phi(n)) = \floor{l_k(n)/6}$ and $(l_k(\phi(n)) -1)$ is not a multiple of $3$. So $b_k(\phi(n)) \geq b_{k_2}(\phi(n))$. The same reasoning as in (a) yields $\phi(n) \in C_\delta \cup D_{\delta} \cup E^T$.

	 We define $B_{\epsilon,l_0}^T = \{ n: n \in B_{\epsilon}^T , l_k(n) \geq l_0 \}$, and we have that $|B_{\epsilon}^T| \leq l_0 +  |B_{\epsilon,l_0}^T|$. We have defined a mapping $\phi$ from $B_{\epsilon,l_0}^T$ to $C_{\delta} \cup D_{\delta} \cup E^T$. To calculate the size of $B_{\epsilon,l_0}^T$, we decompose it according to the value of $\phi$. Namely:
	\eq{
	\{ n: n \in B_{\epsilon,l_0}^T , l_k(n) \geq l_0 \} = \cup_{n^\prime \in  C_{\delta} \cup D_{\delta} \cup E^T} \{ n: n \in B_{\epsilon,l_0}^T , \phi(n) = n^\prime\}.
	}
 Consider $n^\prime$ fixed. If $n \in B_{\epsilon,l_0}^T$ and $\phi(n) = n^\prime$, then $\floor{l_k(n)/6} \in \{ t_{k,k_1}(n^\prime), t_{k,k}(n^\prime) \}$ and $l_k(n)$ is incremented at time $n$ because $L(n) = k$. Therefore:
 \eq{
 | \{ n: n \in B_{\epsilon,l_0}^T , \phi(n) = n^\prime\} | \leq 12.
 }
	Using a union bound we obtain the announced result:
		\eq{
		|B_{\epsilon}^T| \leq  l_0 +  |B_{\epsilon,l_0}^T| \leq   O(1) + 12  ( |C_{\delta}| +  |D_{\delta}| + |E^T|).
	}

\medskip
\noindent	
\underline{Bound on $\mathbb{E} |C_\delta|$.} Observe that for $\delta$ small enough, $C_{2} \subset C_{\delta,1}$, thus we just show that $\EE|C_{\delta,1}|<\infty $. To this aim, we apply Lemma~\ref{lem:deviation} with $\Lambda(s) = \{ n: L(n)=k, l_k(n) = s \}$, and $\Lambda = \cup_{s\ge 1}\Lambda(s)$. Then of course, $|\Lambda(s)| \leq 1$ for all $s$. Moreover by design, $t_{k}(n) \geq s/3$ when $n \in \Lambda(s)$, so we can choose any $\epsilon < 1/3$ in Lemma~\ref{lem:deviation}. Now $C_{\delta,1}=\{n\in \Lambda: | \hat{\mu}_k(n) - \theta_k r_k | > \delta  \}$. From (\ref{eq:ineq3}), we get: $\EE|C_{\delta,1}| < \infty$, and hence $\EE|C_{\delta}| < \infty$.

\medskip
\noindent
\underline{Bound on $\mathbb{E} |D_{\delta} |$.}
Let $k^\prime\in \{k_1,k\}$. Define for any $s$, $\Lambda(s) = \{ n : L(n)=k, k(n) = k^\prime , t_{k^\prime}(n) = s \}$, and $\Lambda=\cup_{s\ge 1}\Lambda(s)$. We have $|\Lambda(s)| \leq 1$, and for any $n\in \Lambda(s)$, $t_{k^\prime}(n)=s \ge \epsilon s$ for any $\epsilon <1$. We can now apply Lemma~\ref{lem:deviation} (where $k$ is replaced by $k^\prime$). Note that $D_{\delta} = \{n\in \Lambda: | \hat{\mu}_{k^\prime}(n) - \theta_{k^\prime} r_{k^\prime} | > \delta\}$, and hence (\ref{eq:ineq3}) leads to $\EE| D_{\delta,k^\prime}| <\infty$, and thus $\EE| D_{\delta}| <\infty$.

\medskip
\noindent
\underline{Bound on $\mathbb{E} |E^T |$.} 
We can show as in~\cite{garivier2011} (the analysis of KL-UCB) that $\mathbb{E}|E^T| = O(\log(\log(T)))$ (more precisely, this result is a simple application of Theorem 10 in ~\cite{garivier2011}). 

We have shown that $\mathbb{E} |B_{\epsilon}^T| = O(\log(\log(T)))$, and hence $\mathbb{E}[l_k(T)]=O(\log(\log(T)))$, which concludes the proof of Theorem \ref{lemma:l1bound}.
\ep



	
